Sketchy: Memory-efficient Adaptive Regularization with Frequent Directions

Adaptive regularization methods that exploit more than the diagonal entries exhibit state of the art performance for many tasks, but can be prohibitive in terms of memory and running time. We find the spectra of the Kronecker-factored gradient covariance matrix in deep learning (DL) training tasks are concentrated on a small leading eigenspace that changes throughout training, motivating a low-rank sketching approach. We describe a generic method for reducing memory and compute requirements of maintaining a matrix preconditioner using the Frequent Directions (FD) sketch. While previous approaches have explored applying FD for second-order optimization, we present a novel analysis which allows efficient interpolation between resource requirements and the degradation in regret guarantees with rank $k$: in the online convex optimization (OCO) setting over dimension $d$, we match full-matrix $d^2$ memory regret using only $dk$ memory up to additive error in the bottom $d-k$ eigenvalues of the gradient covariance. Further, we show extensions of our work to Shampoo, resulting in a method competitive in quality with Shampoo and Adam, yet requiring only sub-linear memory for tracking second moments.

==> NeurIPS/parameter_free.tex <==
\section{Parameter-free Algorithm}\xc{In progress}\label{sec:param-free}
\texttt{S-AdaGrad} (Algorithm \ref{alg:AdaGrad}) with \texttt{FD-Update} (Algorithm \ref{alg:dfd}) includes a learning rate $\eta$ that needs to be tuned according to quantities that are unknown a priori, such as $\tr(G_T^{1/2})$ and $\rho_{1:T}$. It is therefore desirable to adapt to the best learning rate and have a parameter-free algorithm. To this end, we use techniques developed in \citet{param_free_AdaGrad} as a black-box in addition to frequent directions sketching. The resulting guarantee is in general incomparable to the standard AdaGrad guarantee, and there exist problems where either one of them could be better than the other.

\begin{lemma} [Theorem 7 in \cite{param_free_AdaGrad}]
Define $\|\cdot\|_t$ to be $\|x\|_t^2 = x^\top (I + \tilde{G}_t)^{1/2}x$, where $\tilde{G}_t$ is defined to be the same as in  Algorithm \ref{alg:AdaGrad}. Assume $\|g_t\|_{t-1, *} \le 1$ for all $t \in [T]$, where $\|\cdot\|_{t-1, *}$ is the dual norm of $\|\cdot\|_{t-1}$.  Then for any comparator $x^*\in \mathbb{R}^d$, the regret of Algorithm 1 with convexity parameter $\sigma=1$ in \cite{param_free_AdaGrad} with the given sequence of norms $\|\cdot\|_t$ is bounded by 
\[
R_T(x^*) \le \tilde{O}(\sqrt{(\|x^*\|_2^2 + (x^*)^\top G_T^{1/2}x^*)\tr(G_T^{1/2})})
\]
\end{lemma}

Let $\|x\|_A$ denote the matrix norm $\sqrt{x^\top Ax}$, the algorithm is given below for completeness.
\begin{algorithm}[h!]
\caption{\texttt{Parameter-free S-AdaGrad}, Algorithm 1 in \cite{cutkosky2019matrix}}
\begin{algorithmic}[1]
\STATE Instantiate one-dimensional parameter-free online learning algorithm $\A$, see \cite{cutkosky2019matrix}.
\STATE Set $\psi_0(x) = \frac{1}{\sqrt{2}}\|x\|_2^2$, and $w_1 = \text{argmin}_w \psi_0(w) = 0.$
\FOR{$t=1,\dots,T$}
\STATE Get $y_t \in \R$ from $\A$.
\STATE Play $x_t = y_tw_t$, receive $g_t$.
\STATE Set
\begin{align*}
&\psi_t(w) = 
\frac{1}{\sqrt{2}}\|w\|_t^2 \sqrt{1 + \sum_{i=1}^t\|g_i\|_{(I + \tilde{G}_i)^{-1/2}}^2},\ \\
&\text{if }\|w\|_t \le 1,\ \ \text{and }
\infty,\ \text{otherwise}
\end{align*}
\STATE Set $w_{t+1} = \text{argmin}_w \psi_t(w) + \sum_{i=1}^t \langle g_i, w\rangle.$
\STATE Send $s_t = \langle g_t, w_t\rangle$ to $\A$ as the next loss.
\ENDFOR
\end{algorithmic}
\end{algorithm}
